Mind the wealth gap: a new allocation method to match micro and macro statistics for household wealth

The financial and economic crisis recently experienced by many European countries has increased demand for timely, coherent and consistent distributional information for the household sector. In the Euro area, most of the NCBs collect such information through income and wealth surveys, which are often used to inform their decisions. These surveys, however, can often suffer from biases, usually caused by non-response and under-reporting behaviours, leading to a mismatch with macroeconomic aggregates. In this paper, we develop a novel allocation method which combines information from a power law (Pareto) model and imputation procedures so to address these issues simultaneously, when only limited external information is available. We provide two important contributions: first, we adjust the weights of observed survey households for non-response bias, then, we correct for measurement error. Finally, we produce distributional indicators for four Euro-Area countries.

==> changes_from_v1.tex <==
1. Table 1 updated with new Finland results

2. Table 1 updated with new Finland results

3. Figure 2 updated with new Finland results

(just copy paste updated tables and add new figure to new file) 

==> tableBootstrap.tex <==


\begin{center}
\begin{longtable}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]} 
\caption{The missing gap: bootstrap results \label{tabBootstrap}} \\ \toprule


 & \multicolumn{8}{c}{Wealth Shares}\\
 & {Top 1\%} & {Top 5\%}  & {Top 10\%}  & {Top 20\%}  & {Bot 50\%} & {Gini} & {Tail $\alpha$} & {S.r.}  \\
Country & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} \\ 
\midrule
\endhead
& \multicolumn{8}{c}{Base Survey} \\

IT & 0.112298396682892 & 0.291829099334318 & 0.422939876606357 & 0.597363947679912 & 0.103221748181796 & 0.597257827602255 & 1.85989140848314 & --  \\
& (00.074043924) & (0.032349375) & (0.020676699) & (0.012581805) & (0.038947602) & (0.01230447) & (0.074651195) & \\

FR & 0.168214085937998 & 0.351975354033159 & 0.484834150023367 & 0.654808523099853 & 0.0732843123977597 & 0.654630375993903 & 1.76803669448715 & --  \\
& (0.089322942) & (0.036388704) & (0.021976953) & (0.011554199) & (0.039716146) & (0.011225063) & (0.052288883) & \\

DE & 0.21935052933075 & 0.439215812111584 & 0.572874984247392 & 0.742220501700381 & 0.0304273138615544 & 0.739429791137665 & 1.57539435864675 & -- \\
& (0.111291626) & (0.049686226) & (0.030760529) & (0.015098774) & (0.072603913) & (0.013842171) & (0.159378921) & \\

FI  & 0.119671572450594 & 0.285496195960408 & 0.415926382513164 & 0.594781362546254 & 0.100895519188506 & 0.596475653975504 & 2.16217760136116 & -- \\
& (0.050382835) & (0.018772414) & (0.011529657) & (0.006889984) & (0.025254053) & (0.007033199) & (0.068581422) & \\

& \multicolumn{8}{c}{Survey \& missing tail} \\


IT & 0.232531486091024 & 0.390489451785682 & 0.503784569798273 & 0.653921877162636 & 0.0890355086541018 & 0.653026882881629 & 1.47255971252272 & 0.999 \\
& (0.140352891) & (0.068805967) & (0.044394832) & (0.024330073) & (0.056430522) & (0.019044346) & (0.015357159) & \\

FR & 0.217407999911793 & 0.390557528684099 & 0.515535691161499 & 0.675384985462861 & 0.0689360849208009 & 0.673443760931926 & 1.49456340925287 & 1.000 \\
& (0.25414802) & (0.110739881) & (0.066960475) & (0.03445033) & (0.078570837) & (0.020877417) & (0.030471995) & \\

DE & 0.332450500325192 & 0.521587409259061 & 0.635757966259701 & 0.780191887790335 & 0.0259859456714038 & 0.777759947533996 & 1.35119945961989 & 0.971 \\
& (0.077118545) & (0.037726654) & (0.02430974) & (0.012291083) & (0.073533691) & (0.011802833) & (0.017136201) & \\

FI & 0.139426848572624 & 0.301590781394163 & 0.429105534412453 & 0.603927199037159 & 0.0986253402220925 & 0.605582965932978 & 1.6909794945047 & 1.000 \\
& (0.071817044) & (0.026250988) & (0.015714254) & (0.008674642) & (0.026563672) & (0.00876459) & (0.039229624) & \\

& \multicolumn{8}{c}{Pareto-calibration \& missing tail} \\

IT & 0.262273154904489 & 0.429167389770923 & 0.540526035989084 & 0.682935814860495 & 0.0807905953857924 & 0.679527545974163 & 1.47255971252272 & 0.999 \\
& (0.087269404) & (0.043929358) & (0.028611299) & (0.014907495) & (0.045318048) & (0.013948789) & (0.015357159) & \\  

FR & 0.25549516080225 & 0.424415620183047 & 0.545348444211364 & 0.69850016305799 & 0.0614091654920273 & 0.697463084867092 & 1.50900765755787 & 1.000 \\
& (0.181652505) & (0.083733685) & (0.050389792) & (0.024677847) & (0.038990646) & (0.023211861) & (0.029178852) & \\

DE & 0.350837548293654 & 0.53935291250852 & 0.650711271552031 & 0.790511181772615 & 0.024361526046605 & 0.787079960253533 & 1.35119945961989 & 0.971 \\
& (0.083589631) & (0.039739964) & (0.023516879) & (0.010000952) & (0.070521832) & (0.01039992) & (0.017136201) & \\

FI  & 0.19394227565997 & 0.352787332355495 & 0.474545145109581 & 0.637838883115444 & 0.0895781978676136 & 0.637468102808676 & 1.6909794945047 & 1.000 \\
& (0.164869007) & (0.075492925) & (0.046222362) & (0.022306239) & (0.029968827) & (0.019608429) & (0.039229624) & \\ 

& \multicolumn{8}{c}{Par-cal, Proportional allocation \& missing tail} \\

IT & 0.260276891812275 & 0.42757877010625 & 0.53924508969239 & 0.682045003334446 & 0.0809980535960086 & 0.678649465320919 & 1.51086889911487 & 0.999 \\
& (0.10791799) & (0.054076974) & (0.035016892) & (0.018325945) & (0.048250771) & (0.017345783) & (0.009200605) & \\

FR & 0.265499870697547 & 0.431898330893034 & 0.550274747398718 & 0.70046916641588 & 0.062617782351861 & 0.699403975784549 & 1.51920390860791 & 0.996 \\
& (0.18129983) & (0.085520974) & (0.052837983) & (0.027007022) & (0.048272211) & (0.025463006) & (0.032084263) & \\ 

DE & 0.34886843349317 & 0.537941815721212 & 0.649648717367596 & 0.78988111258972 & 0.0244309640373595 & 0.786439108736005 & 1.35255478562493 & 0.971 \\ 
& (0.092227307) & (0.043820285) & (0.025985923) & (0.011021125) & (0.070916238) & (0.011560138) & (0.016247937) & \\

FI & 0.197289014763024 & 0.355497797980354 & 0.476746286201043 & 0.639355643006421 & 0.0891971629463893 & 0.638990938742644 & 1.69455329393991 & 1.000 \\
& (0.171791997) & (0.079373743) & (0.048710654) & (0.023626459) & (0.030878846) & (0.020948357) & (0.039096703) & \\ 

&\\
&\\

& \multicolumn{8}{c}{Par-cal, Single-iteration approach \& missing tail} \\

IT & 0.299058587419332 & 0.463110976875205 & 0.569287879865652 & 0.704598285095509 & 0.0755065533855119 & 0.699485561738833 & 1.49605201772985 & 0.984 \\
& (0.225486224) & (0.117403392) & (0.077133026) & (0.042237522) & (0.102170295) & (0.041774632) & (0.009196682) & \\

FR & 0.266091978897097 & 0.430534084218339 & 0.549683733132177 & 0.701289218891424 & 0.0626294807124399 & 0.699839017778423 & 1.5291974729417 & 0.988 \\
& (0.229959407) & (0.110774328) & (0.067829808) & (0.033365981) & (0.067739478) & (0.033046372) & (0.033996809) & \\

DE & 0.350068046477379 & 0.537985310444823 & 0.649764139295814 & 0.789874190897525 & 0.0243992504664171 & 0.786418844916894 & 1.35294869703719 & 0.97 \\
& (0.084869232) & (0.045522824) & (0.030377721) & (0.015828329) & (0.079638546) & (0.014616543) & (0.01611418) & \\

FI & 0.193421263703285 & 0.353204086550564 & 0.475738613158031 & 0.640201461724536 & 0.0879853641212009 & 0.639697149608628 & 1.70390281930204 & 1.000 \\
& (0.167844416) & (0.084166918) & (0.056439226) & (0.031979879) & (0.049493716) & (0.027975696) & (0.038684284
) & \\ 
    
    
& \multicolumn{7}{c}{Par-cal, Wealth/portfolio calibration, \& missing tail} \\

IT  & 0.272577511378923 & 0.468612967984633 & 0.578396316733653 & 0.711609543937861 & 0.071733962586461 & 0.706079829289487 & 1.49719344631173 & 0.983 \\
& (0.296798357) & (0.121360125) & (0.076636548) & (0.042065957) & (0.110417105) & (0.042278155) & (0.009143348) & \\

FR & 0.224186329759553 & 0.40362461444482 & 0.528726192978709 & 0.687157390568453 & 0.0682581013874622 & 0.683689244680523 & 1.54270049369122 & 0.987 \\
& (0.245881102) & (0.104212265) & (0.059169995) & (0.026051977) & (0.070896338) & (0.026391168) & (0.038278876) & \\

DE & 0.342518499054887 & 0.531316683055971 & 0.645182570424178 & 0.786911473949062 & 0.0255282674003425 & 0.783008677316046 & 1.35358290123553 & 0.942 \\  & (0.114989255) & (0.050432023) & (0.031934494) & (0.016388484) & (0.090627147) & (0.015674941) & (0.020903145) & \\

FI & 0.146750655272949 & 0.321037088014337 & 0.448223817646621 & 0.620326397800795 & 0.0956864466563065 & 0.618250375584804 & 1.7338249343126 & 0.992 \\
& (0.109527528) & (0.043780021) & (0.028971436) & (0.01681636) & (0.031674222) & (0.0125746) & (0.02869323) & \\ 

& \multicolumn{7}{c}{Simultaneous approach} \\

IT & 0.263653207789018 & 0.444637906769167 & 0.560589541083036 & 0.701915303936126 & 0.0802094667536258 & 0.688460422403703 & 1.47620722258654 & 0.999 \\
& (0.080747521) & (0.038100521) & (0.023442986) & (0.013136038) & (0.055437696) & (0.013130281) & (0.005709876) & \\

FR  & 0.264214903014578 & 0.435611392040708 & 0.552546361442613 & 0.698036642995031 & 0.0758410075587718 & 0.692877020230501 & 1.48221595077674 & 0.996 \\
& (0.148302721) & (0.065476277) & (0.040231525) & (0.020834759) & (0.044095909) & (0.018487718) & (0.018619528) & \\

DE & 0.323973885964064 & 0.510471570343241 & 0.625643961065891 & 0.769069025472083 & 0.0342960649580191 & 0.765151672842515 & 1.37337286205768 & 0.97 \\
& (0.09207948) & (0.042801025) & (0.025120159) & (0.011536941) & (0.068353716) & (0.012167132) & (0.018151911) & \\

FI & 0.170695027143761 & 0.337659301792081 & 0.468122540293953 & 0.640058218150101 & 0.0891389310727078 & 0.634309200961399 & 1.77978993993793 & 0.999 \\
& (0.114902346) & (0.048577984) & (0.033591862) & (0.020074588) & (0.049705703) & (0.017467699) & (0.016293128) & \\ 
\bottomrule
\end{longtable} \end{center}
\begin{tabular}{p{\textwidth}}
\small \textit{Notes:} Coefficients of variation reported in parenthesis. Wealth share by percentile, Gini inequality coefficients and Pareto tail parameters for Italy, France, Germany and Finland, estimated using different adjustments for the HFCS data, and accounting for the unobserved part of the Pareto tail. Survey weights are replaced by bootstrap weights. Success rates (S.r.) report the observed probability of convergence for calibration.
\end{tabular}


==> tableBootstrap0.tex <==


\begin{table}[bht!]
\caption{The missing gap: bootstrap results \label{tabBootstrap0}}
\begin{center}
\begin{tabular}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]} \hline \hline

 & \multicolumn{8}{c}{Wealth Shares}\\
 & {Top 1\%} & {Top 5\%}  & {Top 10\%}  & {Top 20\%}  & {Bot 50\%} & {Gini} & {Tail $\alpha$} & {S.r.}  \\
Country & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} \\ 
\hline

& \multicolumn{8}{c}{Pareto-calibration \& missing tail} \\

IT & 0.262273154904489 & 0.429167389770923 & 0.540526035989084 & 0.682935814860495 & 0.0807905953857924 & 0.679527545974163 & 1.47255971252272 & 0.999 \\  & (0.0228884219136773) & (0.018853047741044) & (0.0154651522495527) & (0.0101808620591069) & (0.00366127208948378) & (0.00947858636254179) & (0.0226143334083809) & \\  
FR & 0.25549516080225 & 0.424415620183047 & 0.545348444211364 & 0.69850016305799 & 0.0614091654920273 & 0.697463084867092 & 1.50900765755787 & 1.000 \\  & (0.0464113358980215) & (0.0355378837667567) & (0.0274799949225234) & (0.0172374804394626) & (0.00239438301291377) & (0.0161894161453546) & (0.0440311104585431) & \\
DE & 0.350837548293654 & 0.53935291250852 & 0.650711271552031 & 0.790511181772615 & 0.024361526046605 & 0.787079960253533 & 1.35119945961989 & 0.971 \\  & (0.0293263811106708) & (0.0214338655156781) & (0.0153026979287372) & (0.00790586442205833) & (0.00171801944948326) & (0.00818556879189601) & (0.0231544259891381) & \\
FI  & 0.19394227565997 & 0.352787332355495 & 0.474545145109581 & 0.637838883115444 & 0.0895781978676136 & 0.637468102808676 & 1.6909794945047 & 1.000 \\  & (0.0319750703167327) & (0.0266329477897268) & (0.0219345977128825) & (0.0142277863911386) & (0.00268455349944047) & (0.0124997481058357) & (0.0663364903251033) & \\ 

& \multicolumn{8}{c}{Par-cal, Proportional allocation \& missing tail} \\

IT & 0.260276891812275 & 0.42757877010625 & 0.53924508969239 & 0.682045003334446 & 0.0809980535960086 & 0.678649465320919 & 1.51086889911487 & 0.999 \\  & (0.02808855898802) & (0.0231221661802128) & (0.0188826871343552) & (0.0124991194731679) & (0.00390821852559543) & (0.0117717063818291) & (0.0139009074946235) & \\
FR & 0.265499870697547 & 0.431898330893034 & 0.550274747398718 & 0.70046916641588 & 0.062617782351861 & 0.699403975784549 & 1.51920390860791 & 0.996 \\  & (0.0481350814622234) & (0.0369363657881905) & (0.0290754080233797) & (0.018917586358907) & (0.00302269878472295) & (0.0178089278379667) & (0.0487425380754957) & \\ 
DE & 0.34886843349317 & 0.537941815721212 & 0.649648717367596 & 0.78988111258972 & 0.0244309640373595 & 0.786439108736005 & 1.35255478562493 & 0.971 \\  & (0.0321751962809782) & (0.0235727637788188) & (0.0168817217335733) & (0.00870537877176082) & (0.00173255205591779) & (0.00909134454929226) & (0.0219762246464336) & \\
FI & 0.197289014763024 & 0.355497797980354 & 0.476746286201043 & 0.639355643006421 & 0.0891971629463893 & 0.638990938742644 & 1.69455329393991 & 1.000 \\  & (0.0338926739105535) & (0.0282171909083663) & (0.0232226232645322) & (0.0151057099322489) & (0.00275430546771583) & (0.0133858104159941) & (0.066251446035298) & \\ 


& \multicolumn{8}{c}{Par-cal, Wealth calibration \& missing tail} \\

IT & 0.299058587419332 & 0.463110976875205 & 0.569287879865652 & 0.704598285095509 & 0.0755065533855119 & 0.699485561738833 & 1.49605201772985 & 0.984 \\  & (0.067433591754583) & (0.0543707994879401) & (0.0439108966535908) & (0.0297604857974769) & (0.0077145268557039) & (0.0292207520831415) & (0.0137587146137207) & \\
FR & 0.266091978897097 & 0.430534084218339 & 0.549683733132177 & 0.701289218891424 & 0.0626294807124399 & 0.699839017778423 & 1.5291974729417 & 0.988 \\  & (0.0611903536963754) & (0.0476921238143342) & (0.0372849422862682) & (0.0233992025674304) & (0.00424248834459561) & (0.0231271405271691) & (0.0519878347545169) & \\
DE & 0.350068046477379 & 0.537985310444823 & 0.649764139295814 & 0.789874190897525 & 0.0243992504664171 & 0.786418844916894 & 1.35294869703719 & 0.97 \\  & (0.0297100062600827) & (0.0244906106173175) & (0.0197383538487935) & (0.012502388344085) & (0.00194312082509192) & (0.011494724990738) & (0.0218016594940211) & \\
FI & 0.193421263703285 & 0.353204086550564 & 0.475738613158031 & 0.640201461724536 & 0.0879853641212009 & 0.639697149608628 & 1.70390281930204 & 1.000 \\  & (0.0324646790655563) & (0.0297280992236903) & (0.0268503190059066) & (0.0204735653275346) & (0.00435472259128193) & (0.0178959727253149) & (0.0659142601644852) & \\ 
    
    
& \multicolumn{7}{c}{Par-cal, Wealth/portfolio calibration, \& missing tail} \\

IT  & 0.272577511378923 & 0.468612967984633 & 0.578396316733653 & 0.711609543937861 & 0.071733962586461 & 0.706079829289487 & 1.49719344631173 & 0.983 \\  & (0.080900557419767) & (0.0568709283934349) & (0.0443262969759397) & (0.0299345366027551) & (0.00792065644516152) & (0.0298517521824075) & (0.0136893608682511) & \\
FR & 0.224186329759553 & 0.40362461444482 & 0.528726192978709 & 0.687157390568453 & 0.0682581013874622 & 0.683689244680523 & 1.54270049369122 & 0.987 \\  & (0.0551231817138261) & (0.0420626352731468) & (0.0312847262351819) & (0.0179018087742682) & (0.00483924941809358) & (0.0180433580524761) & (0.0590528409406759) & \\
DE & 0.342518499054887 & 0.531316683055971 & 0.645182570424178 & 0.786911473949062 & 0.0255282674003425 & 0.783008677316046 & 1.35358290123553 & 0.942 \\  & (0.0393859468756262) & (0.0267953749967234) & (0.0206035786707229) & (0.0128962860985774) & (0.00231355405493214) & (0.0122736149058765) & (0.0282941394266553) & \\
FI & 0.146750655272949 & 0.321037088014337 & 0.448223817646621 & 0.620326397800795 & 0.0956864466563065 & 0.618250375584804 & 1.7338249343126 & 0.992 \\  & (0.0160732364690936) & (0.0140550104890588) & (0.0129856875937143) & (0.0104316317253392) & (0.00303079374292565) & (0.0077742511282698) & (0.0497490368430903) & \\ 

& \multicolumn{7}{c}{Simultaneous approach} \\

IT & 0.263653207789018 & 0.444637906769167 & 0.560589541083036 & 0.701915303936126 & 0.0802094667536258 & 0.688460422403703 & 1.47620722258654 & 0.999 \\  & (0.021289342881264) & (0.0169409359949344) & (0.013141892491104) & (0.0092203858315055) & (0.00444662801924293) & (0.00903967873562023) & (0.00842896089352584) & \\
FR  & 0.264214903014578 & 0.435611392040708 & 0.552546361442613 & 0.698036642995031 & 0.0758410075587718 & 0.692877020230501 & 1.48221595077674 & 0.996 \\  & (0.0391837891521691) & (0.0285222122536455) & (0.0222297825984152) & (0.0145434255758916) & (0.00334427818856532) & (0.012809714935957) & (0.0275981607664865) & \\
DE & 0.323973885964064 & 0.510471570343241 & 0.625643961065891 & 0.769069025472083 & 0.0342960649580191 & 0.765151672842515 & 1.37337286205768 & 0.97 \\  & (0.0298313468047436) & (0.0218487066010225) & (0.0157162756121546) & (0.00887270406581787) & (0.00234426346906959) & (0.00930970171467536) & (0.0249293424731844) & \\
FI & 0.170695027143761 & 0.337659301792081 & 0.468122540293953 & 0.640058218150101 & 0.0891389310727078 & 0.634309200961399 & 1.77978993993793 & 0.999 \\  & (0.019613258999234) & (0.0164028082555208) & (0.0157251076432529) & (0.0128489047515883) & (0.00443071325746666) & (0.0110799222005056) & (0.0289983458913939) & \\ 



\hline \hline

\end{tabular}
\end{center}

     {\textit{Notes:} Standard errors reported in parenthesis. Wealth share by percentile, Gini inequality coefficients and Pareto tail parameters for Italy, France, Germany and Finland, estimated using different adjustments for the HFCS data, and accounting for the unobserved part of the Pareto tail. Survey weights are replaced by bootstrap weights. Success rates (S.r.) report the observed probability of convergence for calibration.}


\end{table}

==> tableBootstrap_sd_.tex <==


\begin{center}
\begin{longtable}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.07\textwidth]} 
\caption{The missing gap: bootstrap results \label{tabBootstrapsd}} \\ \toprule


 & \multicolumn{8}{c}{Wealth Shares}\\
 & {Top 1\%} & {Top 5\%}  & {Top 10\%}  & {Top 20\%}  & {Bot 50\%} & {Gini} & {Tail $\alpha$} & {S.r.}  \\
Country & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} \\ 
\midrule

& \multicolumn{8}{c}{Base Survey} \\

IT & 0.112298396682892 & 0.291829099334318 & 0.422939876606357 & 0.597363947679912 & 0.103221748181796 & 0.597257827602255 & 1.85989140848314 & --  \\  & (0.00831501399931371) & (0.00944048888056749) & (0.00874500034819532) & (0.00751591696086528) & (0.0040202395970921) & (0.00734894075824981) & (0.138843115891934) & \\

FR & 0.168214085937998 & 0.351975354033159 & 0.484834150023367 & 0.654808523099853 & 0.0732843123977597 & 0.654630375993903 & 1.76803669448715 & --  \\  & (0.0150253770515391) & (0.0128079270493076) & (0.0106551775310571) & (0.00756578800277312) & (0.00291057048539939) & (0.00734826711257252) & (0.0924486634511387) & \\

DE & 0.21935052933075 & 0.439215812111584 & 0.572874984247392 & 0.742220501700381 & 0.0304273138615544 & 0.739429791137665 & 1.57539435864675 & -- \\  & (0.0244118771766824) & (0.0218229760967007) & (0.017621937434739) & (0.0112066193864131) & (0.00220914203530638) & (0.0102353138733552) & (0.251084652597029) & \\

FI  & 0.119671572450594 & 0.285496195960408 & 0.415926382513164 & 0.594781362546254 & 0.100895519188506 & 0.596475653975504 & 2.16217760136116 & -- \\  & (0.00602939308519984) & (0.00535945291061827) & (0.0047954886577221) & (0.00409803402579515) & (0.00254802082462265) & (0.00419513222603796) & (0.14828521535503) & \\

& \multicolumn{8}{c}{Survey \& missing tail} \\


IT & 0.232531486091024 & 0.390489451785682 & 0.503784569798273 & 0.653921877162636 & 0.0890355086541018 & 0.653026882881629 & 1.47255971252272 & 0.999 \\  & (0.0326364662543248) & (0.0268680045142895) & (0.0223654314376223) & (0.0159099672285989) & (0.0050243202358334) & (0.01243646973674) & (0.0226143334083809) & \\

FR & 0.217407999911793 & 0.390557528684099 & 0.515535691161499 & 0.675384985462861 & 0.0689360849208009 & 0.673443760931926 & 1.49456340925287 & 1.000 \\  & (0.0552538126721357) & (0.043250294224797) & (0.0345205147441461) & (0.0232672359175313) & (0.00541636585910231) & (0.0140597661231863) & (0.0455423290617374) & \\

DE & 0.332450500325192 & 0.521587409259061 & 0.635757966259701 & 0.780191887790335 & 0.0259859456714038 & 0.777759947533996 & 1.35119945961989 & 0.971 \\  & (0.0256380987912994) & (0.0196777476977122) & (0.0154551109564347) & (0.00958940305330507) & (0.00191084248826413) & (0.00917977068777638) & (0.0231544259891381) & \\

FI & 0.139426848572624 & 0.301590781394163 & 0.429105534412453 & 0.603927199037159 & 0.0986253402220925 & 0.605582965932978 & 1.6909794945047 & 1.000 \\  & (0.0100132240851909) & (0.00791705591074159) & (0.00674307318443821) & (0.0052388523237938) & (0.00261985115990621) & (0.00530768631836894) & (0.0663364903251033) & \\

& \multicolumn{8}{c}{Pareto-calibration \& missing tail} \\

IT & 0.262273154904489 & 0.429167389770923 & 0.540526035989084 & 0.682935814860495 & 0.0807905953857924 & 0.679527545974163 & 1.47255971252272 & 0.999 \\  & (0.0228884219136773) & (0.018853047741044) & (0.0154651522495527) & (0.0101808620591069) & (0.00366127208948378) & (0.00947858636254179) & (0.0226143334083809) & \\  
FR & 0.25549516080225 & 0.424415620183047 & 0.545348444211364 & 0.69850016305799 & 0.0614091654920273 & 0.697463084867092 & 1.50900765755787 & 1.000 \\  & (0.0464113358980215) & (0.0355378837667567) & (0.0274799949225234) & (0.0172374804394626) & (0.00239438301291377) & (0.0161894161453546) & (0.0440311104585431) & \\
DE & 0.350837548293654 & 0.53935291250852 & 0.650711271552031 & 0.790511181772615 & 0.024361526046605 & 0.787079960253533 & 1.35119945961989 & 0.971 \\  & (0.0293263811106708) & (0.0214338655156781) & (0.0153026979287372) & (0.00790586442205833) & (0.00171801944948326) & (0.00818556879189601) & (0.0231544259891381) & \\
FI  & 0.19394227565997 & 0.352787332355495 & 0.474545145109581 & 0.637838883115444 & 0.0895781978676136 & 0.637468102808676 & 1.6909794945047 & 1.000 \\  & (0.0319750703167327) & (0.0266329477897268) & (0.0219345977128825) & (0.0142277863911386) & (0.00268455349944047) & (0.0124997481058357) & (0.0663364903251033) & \\ 

& \multicolumn{8}{c}{Par-cal, Proportional allocation \& missing tail} \\

IT & 0.260276891812275 & 0.42757877010625 & 0.53924508969239 & 0.682045003334446 & 0.0809980535960086 & 0.678649465320919 & 1.51086889911487 & 0.999 \\  & (0.02808855898802) & (0.0231221661802128) & (0.0188826871343552) & (0.0124991194731679) & (0.00390821852559543) & (0.0117717063818291) & (0.0139009074946235) & \\
FR & 0.265499870697547 & 0.431898330893034 & 0.550274747398718 & 0.70046916641588 & 0.062617782351861 & 0.699403975784549 & 1.51920390860791 & 0.996 \\  & (0.0481350814622234) & (0.0369363657881905) & (0.0290754080233797) & (0.018917586358907) & (0.00302269878472295) & (0.0178089278379667) & (0.0487425380754957) & \\ 
DE & 0.34886843349317 & 0.537941815721212 & 0.649648717367596 & 0.78988111258972 & 0.0244309640373595 & 0.786439108736005 & 1.35255478562493 & 0.971 \\  & (0.0321751962809782) & (0.0235727637788188) & (0.0168817217335733) & (0.00870537877176082) & (0.00173255205591779) & (0.00909134454929226) & (0.0219762246464336) & \\
FI & 0.197289014763024 & 0.355497797980354 & 0.476746286201043 & 0.639355643006421 & 0.0891971629463893 & 0.638990938742644 & 1.69455329393991 & 1.000 \\  & (0.0338926739105535) & (0.0282171909083663) & (0.0232226232645322) & (0.0151057099322489) & (0.00275430546771583) & (0.0133858104159941) & (0.066251446035298) & \\ 


& \multicolumn{8}{c}{Par-cal, Wealth calibration \& missing tail} \\

IT & 0.299058587419332 & 0.463110976875205 & 0.569287879865652 & 0.704598285095509 & 0.0755065533855119 & 0.699485561738833 & 1.49605201772985 & 0.984 \\  & (0.067433591754583) & (0.0543707994879401) & (0.0439108966535908) & (0.0297604857974769) & (0.0077145268557039) & (0.0292207520831415) & (0.0137587146137207) & \\
FR & 0.266091978897097 & 0.430534084218339 & 0.549683733132177 & 0.701289218891424 & 0.0626294807124399 & 0.699839017778423 & 1.5291974729417 & 0.988 \\  & (0.0611903536963754) & (0.0476921238143342) & (0.0372849422862682) & (0.0233992025674304) & (0.00424248834459561) & (0.0231271405271691) & (0.0519878347545169) & \\
DE & 0.350068046477379 & 0.537985310444823 & 0.649764139295814 & 0.789874190897525 & 0.0243992504664171 & 0.786418844916894 & 1.35294869703719 & 0.97 \\  & (0.0297100062600827) & (0.0244906106173175) & (0.0197383538487935) & (0.012502388344085) & (0.00194312082509192) & (0.011494724990738) & (0.0218016594940211) & \\
FI & 0.193421263703285 & 0.353204086550564 & 0.475738613158031 & 0.640201461724536 & 0.0879853641212009 & 0.639697149608628 & 1.70390281930204 & 1.000 \\  & (0.0324646790655563) & (0.0297280992236903) & (0.0268503190059066) & (0.0204735653275346) & (0.00435472259128193) & (0.0178959727253149) & (0.0659142601644852) & \\ 
    
    
& \multicolumn{7}{c}{Par-cal, Wealth/portfolio calibration, \& missing tail} \\

IT  & 0.272577511378923 & 0.468612967984633 & 0.578396316733653 & 0.711609543937861 & 0.071733962586461 & 0.706079829289487 & 1.49719344631173 & 0.983 \\  & (0.080900557419767) & (0.0568709283934349) & (0.0443262969759397) & (0.0299345366027551) & (0.00792065644516152) & (0.0298517521824075) & (0.0136893608682511) & \\
FR & 0.224186329759553 & 0.40362461444482 & 0.528726192978709 & 0.687157390568453 & 0.0682581013874622 & 0.683689244680523 & 1.54270049369122 & 0.987 \\  & (0.0551231817138261) & (0.0420626352731468) & (0.0312847262351819) & (0.0179018087742682) & (0.00483924941809358) & (0.0180433580524761) & (0.0590528409406759) & \\
DE & 0.342518499054887 & 0.531316683055971 & 0.645182570424178 & 0.786911473949062 & 0.0255282674003425 & 0.783008677316046 & 1.35358290123553 & 0.942 \\  & (0.0393859468756262) & (0.0267953749967234) & (0.0206035786707229) & (0.0128962860985774) & (0.00231355405493214) & (0.0122736149058765) & (0.0282941394266553) & \\
FI & 0.146750655272949 & 0.321037088014337 & 0.448223817646621 & 0.620326397800795 & 0.0956864466563065 & 0.618250375584804 & 1.7338249343126 & 0.992 \\  & (0.0160732364690936) & (0.0140550104890588) & (0.0129856875937143) & (0.0104316317253392) & (0.00303079374292565) & (0.0077742511282698) & (0.0497490368430903) & \\ 

& \multicolumn{7}{c}{Simultaneous approach} \\

IT & 0.263653207789018 & 0.444637906769167 & 0.560589541083036 & 0.701915303936126 & 0.0802094667536258 & 0.688460422403703 & 1.47620722258654 & 0.999 \\  & (0.021289342881264) & (0.0169409359949344) & (0.013141892491104) & (0.0092203858315055) & (0.00444662801924293) & (0.00903967873562023) & (0.00842896089352584) & \\
FR  & 0.264214903014578 & 0.435611392040708 & 0.552546361442613 & 0.698036642995031 & 0.0758410075587718 & 0.692877020230501 & 1.48221595077674 & 0.996 \\  & (0.0391837891521691) & (0.0285222122536455) & (0.0222297825984152) & (0.0145434255758916) & (0.00334427818856532) & (0.012809714935957) & (0.0275981607664865) & \\
DE & 0.323973885964064 & 0.510471570343241 & 0.625643961065891 & 0.769069025472083 & 0.0342960649580191 & 0.765151672842515 & 1.37337286205768 & 0.97 \\  & (0.0298313468047436) & (0.0218487066010225) & (0.0157162756121546) & (0.00887270406581787) & (0.00234426346906959) & (0.00930970171467536) & (0.0249293424731844) & \\
FI & 0.170695027143761 & 0.337659301792081 & 0.468122540293953 & 0.640058218150101 & 0.0891389310727078 & 0.634309200961399 & 1.77978993993793 & 0.999 \\  & (0.019613258999234) & (0.0164028082555208) & (0.0157251076432529) & (0.0128489047515883) & (0.00443071325746666) & (0.0110799222005056) & (0.0289983458913939) & \\ \bottomrule
\end{longtable} \end{center}
\begin{tabular}{p{\textwidth}}
\small \textit{Notes:} Standard deviation reported in parenthesis. Wealth share by percentile, Gini inequality coefficients and Pareto tail parameters for Italy, France, Germany and Finland, estimated using different adjustments for the HFCS data, and accounting for the unobserved part of the Pareto tail. Survey weights are replaced by bootstrap weights. Success rates (S.r.) report the observed probability of convergence for calibration.
\end{tabular}


==> tableGWfactors_sd_.tex <==

\begin{table}[H]
\caption{Simultaneous approach: final multivariate calibration adjustment factors \label{tabGWfactor}}
\begin{center}
\begin{tabular}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth]
                    } \toprule

 & \multicolumn{10}{c}{Percentile}\\
 & {0.10} & {0.20} & {0.30} & {0.40} & {0.50} & {0.60} & {0.70} & {0.80} & {0.90} & {1.00} \\
Country  & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} & {(9)} & {(10)}\\ 
\midrule

IT & 1.08059479507623 & 1.74513226158673 & 1.90534814783623 & 1.80504851993494 & 1.79590809499743 & 1.80650755989907 & 1.82743252990015 & 1.8319358403669 & 1.87606257634517 & 2.02873973353276 \\
 & (0.893303678683743) & (2.2363833617722) & (2.67322210371137) & (2.58198173050306) & (2.29820464660067) & (2.29367577095453) & (2.2871469010655) & (2.29595063259409) & (2.35220903694556) & (2.78055865204042) \\

FR & 1.54227563589496 & 1.8987480688141 & 3.51680347951392 & 2.26295141332168 & 2.03113588016868 & 2.76144714399457 & 2.5247217458977 & 2.40771632885838 & 3.3433176591973 & 7.39091768288684 \\
& (4.30664361883722) & (10.7991213146797) & (42.1140876926058) & (8.61675971426567) & (7.89612073467603) & (20.3182871117176) & (10.4155763085105) & (4.66722300439004) & (13.2608398623978) & (75.4519930925827) \\

DE & 3.12858863854831 & 3.90962418049958 & 4.36070219537968 & 6.15621875914143 & 4.66281644814334 & 4.59735375300641 & 5.08369683065062 & 5.1159253244696 & 4.5545374007818 & 5.21534410850281 \\
 & (10.3538360235581) & (10.9465754751926) & (11.3211164048597) & (34.6101241368089) & (11.8160925409326) & (15.4180146647553) & (16.9428620202252) & (13.6488908344174) & (11.3379565538221) & (14.0223563591953) \\

FI & 2.23916606530077 & 2.34369904445013 & 2.56645771448216 & 2.04149021941383 & 1.73171005107291 & 1.67170999501747 & 1.80609864319198 & 1.57504768022322 & 1.88165318664616 & 2.52664625621321 \\
 & (5.25778077682922) & (4.9145132464133) & (8.57148509467608) & (3.75803892469482) & (2.85453139126746) & (2.3363706054487) & (4.01487476277348) & (2.12160604093732) & (3.29817929542704) & (4.30386747859667) \\

\bottomrule


\end{tabular}
\end{center}

\begin{tabular}{p{\textwidth}}
\small \textit{Notes:} Mean and standard deviation of overall adjustment factors $a_i$ from the multivariate calibration approach for imputation as a function of gross wealth percentiles.
\end{tabular}

\end{table}


==> tableGfactors_sd_.tex <==

\begin{table}[H]
\caption{Simultaneous approach: final multivariate calibration adjustment factors \label{tabGfactorsd}}
\begin{center}
\begin{tabular}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.056\textwidth]
                    } \toprule

 & \multicolumn{10}{c}{Percentile}\\
 & {0.10} & {0.20} & {0.30} & {0.40} & {0.50} & {0.60} & {0.70} & {0.80} & {0.90} & {1.00} \\
Country  & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} & {(9)} & {(10)}\\ 
\midrule

IT & 1.37026106783785 & 1.94440779863392 & 1.95227702414148 & 1.17050116941896 & 1.08991912100276 & 1.08513143028942 & 1.1194212030138 & 1.14095589716323 & 1.18677959156013 & 1.32643318666427 \\
 & (0.150866397946227) & (0.249635890230271) & (0.362417773836174) & (0.0631898887739853) & (0.0208352985505102) & (0.017875807827956) & (0.0174622584110338) & (0.0247954299059245) & (0.0193111708218208) & (0.129724960644913) \\

FR & 1.03447924352059 & 1.57610743824402 & 2.3873434528838 & 1.75403539163449 & 1.2211060987705 & 1.12997667254321 & 1.12195596456841 & 1.1263329682173 & 1.1337170289553 & 1.23084270910749 \\
& (0.105635136146594) & (0.238402717336025) & (0.159040459408615) & (0.343488825999179) & (0.0572032259764915) & (0.00653112822347182) & (0.00465079788258354) & (0.00756828656051612) & (0.00944911719457452) & (0.138689681439333) \\

DE & 1.1189058940686 & 1.2780136912077 & 1.55871252851926 & 1.71477184319106 & 1.59634852450513 & 1.33869270844707 & 1.17306248428225 & 1.12185249146972 & 1.11040076603235 & 1.09962970264282\\
 & (0.131581445637774) & (0.0984221104239532) & (0.0631979702085511) & (0.0413167132698329) & (0.0684910772474013) & (0.0815389827338701) & (0.0204357829005784) & (0.0107241855258019) & (0.00769727856106052) & (0.018958334030272) \\


FI &  0.943071184741476 & 1.08568515940912 & 1.35001933624595 & 1.10319276719353 & 1.04152778920335 & 1.02804184112081 & 1.03259520309763 & 1.03951978214609 & 1.04670343772154 & 1.0448674536859\\
 & (0.0873255758047087) & (0.098110108972605) & (0.0770002357009329) & (0.0484933830808665) & (0.00475245402672316) & (0.00333510834060752) & (0.00463144711599158) & (0.00264193715216094) & (0.00334678221021083) & (0.030003648503317) \\


\bottomrule


\end{tabular}
\end{center}

\begin{tabular}{p{\textwidth}}
\small \textit{Notes:} Mean and standard deviation of overall adjustment factors $a_i$ from the multivariate calibration approach for imputation as a function of gross wealth percentiles.
\end{tabular}

\end{table}


==> tableTopshares.tex <==


\begin{table}[H]
\caption{The missing gap: distributional wealth indicators \label{tabTShares}}
\begin{center}
\begin{tabular}{lS[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth] S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth]
                    S[table-format=1.3,
                    round-mode=places,
                    round-precision=3, table-number-alignment = center, table-column-width = 0.08\textwidth]} \toprule

 & \multicolumn{7}{c}{Wealth Shares}\\
 & {Top 1\%} & {Top 5\%}  & {Top 10\%}  & {Top 20\%}  & {Bot 50\%} & {Gini} & {Tail $\alpha$}  \\
Country & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} \\ 
\midrule

& \multicolumn{7}{c}{Base Survey} \\

IT & 0.1135414 & 0.2928937 & 0.4237249 & 0.5977503 &  0.1033786 & 0.5971817 & 1.951613 \\
FR & 0.1777410 & 0.3612573 & 0.4942968 & 0.6636282 & 0.06892689 & 0.6630178 & 1.77076 \\
DE & 0.2258016 & 0.4432907 & 0.5754625 & 0.7442643 & 0.03001578 & 0.7410518 & 1.499281 \\
FI & 0.120004015 & 0.28575242 & 0.41621747 & 0.59493453 & 0.1008288 & 0.5964584 & 2.145392 \\ 

& \multicolumn{7}{c}{Survey \& missing tail} \\

IT & 0.2207094 & 0.3794400 & 0.4948255 & 0.6477326 & 0.09074253 & 0.6469042 & 1.490836 \\
FR & 0.1980013 & 0.3772809 & 0.5069829 & 0.6720342 & 0.06719778 & 0.6714585 & 1.537246\\ % 1.536252
DE & 0.3291251 & 0.5197045 & 0.6337345 & 0.7793665 & 0.02597528 & 0.7763417 & 1.361727 \\
FI & 0.1364734 & 0.2989109 & 0.4269752 & 0.6023960 &  0.09894179  & 0.6039581 & 1.717602 \\ 

& \multicolumn{7}{c}{Pareto-calibration \& missing tail} \\

IT & 0.2655057 & 0.4309853 & 0.5403791 & 0.6816255 & 0.08393818 & 0.676523 & 1.456047 \\
FR & 0.2738163 & 0.4375406 & 0.5556797 & 0.7049778 & 0.06097243 & 0.7035584 & 1.499868 \\
DE & 0.3600762 & 0.5478988 & 0.6566814 & 0.7926404 & 0.02471128 & 0.7886409 & 1.364833 \\
FI & 0.1921673 & 0.3503730 & 0.4718573 & 0.6349555 & 0.09130164 & 0.6343717 & 1.717602 \\ 

& \multicolumn{7}{c}{Par-cal, Proportional allocation \& missing tail} \\

IT & 0.2986025 & 0.4704124 & 0.5807633 & 0.7147173 & 0.07749535 & 0.7164887 & 1.427452 \\
FR & 0.2386463 & 0.4078761 & 0.5307819 & 0.6871827 & 0.07023237 & 0.6989841 & 1.557694 \\
DE & 0.3370375 & 0.5169412 & 0.6319117 & 0.7741009 & 0.03251645 & 0.7336069 & 1.375624 \\
FI & 0.1901221 & 0.3485809 & 0.4704004 & 0.6339484 & 0.09155352 & 0.633372 & 1.735287 \\ 

& \multicolumn{7}{c}{Single-iteration approach \& missing tail} \\

IT & 0.3002861 & 0.4645724 & 0.5686188 & 0.7016403 & 0.07837705 & 0.6743792 & 1.442174  \\
FR & 0.2644996 & 0.4283579 & 0.5475698 & 0.6980228 & 0.06323017 & 0.714199  & 1.534188 \\
DE & 0.3568284 & 0.5485280 & 0.6583804 & 0.7946897 & 0.02429046 & 0.7607378 & 1.365316 \\
FI & 0.1881814 & 0.3486941 & 0.4715287 & 0.6360913 & 0.09035164 & 0.6350853 & 1.706971 \\ 

& \multicolumn{7}{c}{Single-iteration approach, portfolio calibration, \& missing tail} \\

IT & 0.3028315 & 0.4699631 & 0.5800269 & 0.7117514 & 0.07284551 & 0.70682 & 1.43162 \\
FR & 0.2442837 & 0.4219004 & 0.5433124 & 0.6951758 & 0.06422416 & 0.6930525 & 1.510868\\
DE & 0.3623710 & 0.5487513 & 0.6579050 & 0.7939098 & 0.02478678 & 0.7894852 & 1.365239 \\
FI & 0.1424634 & 0.3118930 & 0.4394885 & 0.6129370 & 0.09952350 & 0.610366 & 1.778829  \\ 

& \multicolumn{7}{c}{Simultaneous approach} \\

IT & 0.299274833407283 & 0.482612014251461 & 0.595207135420408 & 0.729665691577544 & 0.0693698902724493 & 0.707566217281463 & 1.46462128167641 \\
FR & 0.286843425846978 & 0.454142739500061 & 0.568708037989891 & 0.71031217682572 & 0.0714555067498729 & 0.698281057105233 & 1.50196176761406 \\
DE & 0.34049280728372 & 0.524236685918064 & 0.635677894333435 & 0.77367928588928 & 0.0342466988289143 & 0.766857031286634 & 1.38785073033214 \\
FI & 0.173207758827924 & 0.336311172263858 & 0.460605596531566 & 0.628015237595531 & 0.0969096807261284 & 0.616664243468137 & 1.74836019878326  \\

%& \multicolumn{7}{c}{Simultaneous approach} \\

%IT & 0.298841154086277 & 0.490108900225802 & 0.606789274485056 & 0.73971200634124 & 0.0642527106558823 & 0.732063291300114 & 1.48895689777989 \\
%FR & 0.23432140883185 & 0.405886600726074 & 0.52729550368952 & 0.680961641302046 & 0.0768188950990732 & 0.672941232256357 & 1.5418340555706 \\
%DE & 0.349816513128321 & 0.529258003751151 & 0.639200631727154 & 0.775126534802375 & 0.0351702989450018 & 0.760811595622543 & 1.37144396172923  \\
%FI & 0.284909897821215 & 0.45549201074976 & 0.577143334150622 & 0.724203054397878 & 0.0653100943805962 & 0.7135326148293 & 1.46956177680748  \\

%& \multicolumn{5}{c}{Multivariate classic} \\

%IT &  &  &  &  &  \\
%FR & 0.3297805 & 0.5070243 & 0.6232607 & 0.7559642 & 0.04949932 \\
%DE &  &  &  &  &  \\
%FI &  &  &  &  &  \\

%& \multicolumn{5}{c}{Par-cal, Wealth calibration \& missing tail} \\

%IT & 0.3606379 & 0.5100648 & 0.6073408 & 0.7278989 & 0.07497643 \\
%FR & 0.2215915 & 0.3879796 & 0.5131798 & 0.6730039 & 0.07314748 \\
%DE & 0.3268595 & 0.5068082 & 0.6237689 & 0.7677248 & 0.03415198  \\
%FI & 0.3159118 & 0.4814298 & 0.5921113 & 0.7309323 & 0.06090329 \\ \\

\bottomrule

\end{tabular}
\end{center}

\begin{tabular}{p{\textwidth}}
\small \textit{Notes:} Wealth share by percentile, Gini inequality coefficients and Pareto tail parameters for Italy, France, Germany and Finland, estimated using different adjustments for the HFCS data, and accounting for the unobserved part of the Pareto tail.
\end{tabular}


\end{table}

==> tabletest.tex <==
\begin{table}[H]
\caption{Enter table caption here.\label{tab1}}{%
\begin{tabular}{lccc} \hline \hline

Tap &Relative &Relative &Relative mean\\
number &power (dB) &delay (ns) &power (dB)\\ \hline

3 &0$-9.0$ &68,900\footnotemark[1] &$-12.8$\\
4 &$-10.0$ &12,900\footnotemark[2] &$-10.0$\\
5 &$-15.0$ &17,100 &$-25.2$\\ \hline \hline

\end{tabular}}{\footnotetext[1]{Source: Example for table source text.}
\footnotetext[1]{Example for a first table footnote. Example for a first table footnote.
Example for a first table footnote. Example for a first table footnote.}
\footnotetext[2]{Example for a second table footnote.}}
\end{table}
